Mitigation of Radar Range Deception Jamming Using Random Finite Sets

This paper presents a radar target tracking framework for addressing main-beam range deception jamming attacks using random finite sets (RFSs). Our system handles false alarms and detections with false range information through multiple hypothesis tracking (MHT) to resolve data association uncertainties. We focus on range gate pull-off (RGPO) attacks, where the attacker adds positive delays to the radar pulse, thereby mimicking the target trajectory while appearing at a larger distance from the radar. The proposed framework incorporates knowledge about the spatial behavior of the attack into the assumed RFS clutter model and uses only position information without relying on additional signal features. We present an adaptive solution that estimates the jammer-induced biases to improve tracking accuracy as well as a simpler non-adaptive version that performs well when accurate priors on the jamming range are available. Furthermore, an expression for RGPO attack detection is derived, where the adaptive solution offers superior performance. The presented strategies provide tracking resilience against multiple RGPO attacks in terms of position estimation accuracy and jamming detection without degrading tracking performance in the absence of jamming.

==> manuscript_sections/algorithm_multiple_gaussians.tex <==
%
% -- ALGORITHM 
%

\RestyleAlgo{ruled}
\SetKwComment{Comment}{/* }{ */}
\begin{algorithm}
\caption{Management of the $C_k$ components in $\lambda_{J,k}(\cdot|\bx_k)$~\eqref{eq:multi_intensity_function} to model multiple attacks at time $k$ after the prediction and update steps}\label{alg:proposed_approach}
\KwData{Initial Gaussian component in \textit{vigilant} status and target state vector $\tilde{\bx}_k^{(1)} = [\bp_k^\top, \bv_k^\top, b_k^{(1)}]^\top$}
\KwResult{Gaussian mixture model with components switching between \textit{vigilant}, \textit{active}, and \textit{dormant} statuses}

\For{each component $i = 0, 1, \ldots, C_k$}{
  Retrieve the state index $j$ associated with component $i$: $j = \text{index}(i)$\;
  
  % FIRST IF
  \uIf{$s_k^{(i)}$ is \textit{vigilant}}{


% SECOND IF 
\uIf{$t_{\text{act},k}^{(i)} > T_\text{act}$}{
    $s_k^{(i)} \gets$ \textit{active}\;
          Add a new component $i'$\;
          $s_k^{(i')} \gets$ \textit{vigilant}\;
          $C_k \gets C_k + 1$\;
          $\tilde{\bx}_k^{C_k + 1} \gets [(\tilde{\bx}_k^{C_k})^\top, b_k^{C_k + 1}]^\top$\;
          Renormalize the Gaussian mixture weights\;
          $t_{\text{act},k}^{(i)} \gets t_{\text{act},k}^{(i)} + 1$\;
  }
  % ELSEIF
  \uElseIf{elseif condition}{
    something elseif \;
  }
  %ELSE
  \Else{
    something else \;
  }
    
  }
    \ElseIf{$s_k^{(i)}$ is \textit{active}}{
      % Actions for the new condition
          \If{uncertainty in bias estimation $b_k^i > U_\text{dorm}$ for $T_\text{dorm}$ time steps}{
        Change status of component $i$ to \textit{dormant}\;
        Remove component $i$ from the mixture\;
        Reduce the state vector by removing $b_k^i$\;
        $\tilde{\bx}_k \gets \tilde{\bx}_k \setminus b_k^i$\;
        Adjust mean and covariances of all posterior components\;
        Renormalize the Gaussian mixture weights\;
      }}
  
}
Update the Gaussian mixture components based on new measurements\;
\end{algorithm}
%
